Semantic Resizing of Charts Through Generalization:A Case Study with Line Charts

Inspired by cartographic generalization principles, we present a generalization technique for rendering line charts at different sizes, preserving the important semantics of the data at that display size. The algorithm automatically determines the generalization operators to be applied at that size based on spatial density, distance, and the semantic importance of the various visualization elements in the line chart. A qualitative evaluation of the prototype that implemented the algorithm indicates that the generalized line charts pre-served the general data shape, while minimizing visual clutter. We identify future opportunities where generalization can be extended and applied to other chart types and visual analysis authoring tools.

==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> tex/contribution.tex <==
Inspired by cartographic principles for generalization, this research explores how such best practices can be applied to other types of visualizations when rendering at different scales. In particular, we started our work with line charts, a common visualization type, to determine how the semantics and design principles of line charts could help inform the level of detail rendered at a given scale. In this paper, we make two main contributions:

\begin{tight_itemize}

\item \textbf{Spatial Metrics for Generalization: } We present a set of spatial metrics to examine geometric properties and relationships among the identified elements in a line chart. These spatial metrics is used to determine the presence of visual clutter and complexity in a view to determine the generalization operators. 

\item \textbf{Generalization Techniques for Line Charts: } We have also developed a set of generalization techniques specifically designed to support variable-sized line charts. Using these techniques, the level of detail, and the presence or absence of visual elements can be altered based on their inherent spatial constraints and semantic importance. 

\end{tight_itemize}


==> tex/generalization.tex <==
Line charts comprise a variety of syntactic elements including framing (axis, gridlines, etc.), identifying (labels, etc.), and data-representative marks (points and lines, etc.) \cite{Heer, Kosslyn}. One of the important considerations for successful generalization is how the complexities of a visualization view can be reduced efficiently. In other words, it is very important for generalization techniques to select and retain any elements that include important semantic information, whereas unnecessary details should be reduced. Generally, the importance of semantic information is decided by the underlying values or certain relationships with other elements. We focus on how the generalization maintains this information as the scale is reduced. Our design considerations for generalization techniques emphasize (1) how a visualization at a smaller scale can be simplified while still preserving its essential semantic information consistently, (2) how the semantic information can be employed when we simplify or select elements in a data visualization, and (3) what new representations can be supported to reduce visual clutter and density as scale is reduced. In order to inform the design of a generalization system, we begin by identifying types of high-level generalization tasks for data visualizations with semantic information and view constraints. Each visualization generalization type is supported by one or more low-level generalization operators, which will be explained in Section 3.4.
\subsection{Selection of Syntactic Elements}
The selections process changes the visibility of each syntactic element in a chart. This procedure determines which visual elements should be visible or invisible in a given visualization view, based on certain spatial constraints (section 3.2). For example, as the scale is changed, the visual elements of a visualization are simply added or removed adaptively based on semantic importance and visual clutter constraints. Semantic importance (general data points vs. data points of maximum or minimum values) can be a criterion for identifying an element that should be maintained.  
\subsection{Changes in Detail}
Any changes represent an adjustment to the level of detail and information density according to the scale of visualization. For example, as the size of a line chart is increased, it can show all data points and detail annotations. Conversely, as the size is decreased, the amount of detail for each element is reduced or simplified. Also, any diminished visual quality can be easily overlooked when the scale is smaller. For example, a certain label detail can be changed based on different scales or visual clutter. Each label contains not only data values but also important annotation information if space allows..  
\subsection{Semantic Transitions}
If a syntactic element disappears on one visualization scale, an alternative element containing analogous semantic information should replace it when the visualization scale is altered. This type of generalization means that users do not lose essential information when a visualization is scaled down. For example, if an axis is removed, a simple reference line showing data ranges can be added (Figure x).   
\subsection{Changes in Visual Encodings and Data Schema}
Data representations do not have to be immutable; visual mapping can be altered according to an optimal visibility state of a visualization view. For example, an original bar chart can be replaced with a pie chart for ease of interpretation. When data points on a scatter plot initially created using a computer are too small and dense for users to visualize on a smart phone screen, the data points can be replaced with a heat map. It is also possible to change the data schema being represented by adding or removing dimensions. For example, a bar chart can be replaced with a line chart by adding a time dimension. A bivariate graph can be presented as small multiple displays if data points have too many overlaps.

